Sorting Out Quantum Monte Carlo

Molecular modeling at the quantum level requires choosing a parameterization of the wavefunction that both respects the required particle symmetries, and is scalable to systems of many particles. For the simulation of fermions, valid parameterizations must be antisymmetric with respect to the exchange of particles. Typically, antisymmetry is enforced by leveraging the anti-symmetry of determinants with respect to the exchange of matrix rows, but this involves computing a full determinant each time the wavefunction is evaluated. Instead, we introduce a new antisymmetrization layer derived from sorting, the $\textit{sortlet}$, which scales as $O(N \log N)$ with regards to the number of particles -- in contrast to $O(N^3)$ for the determinant. We show numerically that applying this anti-symmeterization layer on top of an attention based neural-network backbone yields a flexible wavefunction parameterization capable of reaching chemical accuracy when approximating the ground state of first-row atoms and small molecules.

==> attic.tex <==

Existing arguments in  \cite{pfau_ab-initio_2020, pang_on2_2022} have attempted to establish universality of their respective constructions in a pointwise sense, i.e that there is a sequence of neural network ansatz $\psi_n$, that for the ground state $\Psi$, satisfy for each $r \in \R^{3N}$ that $\lim_{r \to \infty} \psi_n(r) = \psi(r)$. In the framework of quantum mechanics, however, this is neither necessary nor sufficient for our target application, which is computing the expected value of observables. Therefore, the goal of this section will not be to show that the sorting ansatz is pointwise universal, but rather prove the following theorem:

\begin{theorem}
\label{thm:univ-energy}
  There is a sequence of smooth sortlets, $\Psi_{\alpha^1}^\ep$ such that
  \begin{equation}
    \ang{\Psi^{\ep}_{\alpha} \vert \hat H \vert \Psi^{\ep}_{\alpha}} \to \ang{\Psi_g \vert \hat H \vert \Psi_g}
  \end{equation}
  This implies that we can approximate the energy arbitrarily well with our sorting ansatz.
\end{theorem}


\begin{proposition}
If we allow $\alpha$ to be non-smooth, we can represent any anti-symmetric function almost everywhere, up to the sign. For any anti-symmetric function $\Psi^g : \R^n \to \R$, there is a discontinuous, permutation equivariant function $\alpha : \R^{3 \times N} \to \R^N$ such that $\Psi_\alpha$ (as defined in \Cref{eq:sortlet}), satisfies $\Psi_\alpha = \pm \Psi_g$ a.e. 
\end{proposition}
\begin{proof}
Define 
\begin{equation}
\alpha(r) = { |\Psi_g|^{1/n} \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i) ]} x(r)
\end{equation}
where $\hat x(q) = \arctan(q_x)$, i.e the function that extracts the $x$ coordinate from $q$ and bounds it using $\arctan$, and the $r_i$ are sorted by $\hat x(r_i)$. Clearly the set 
\begin{equation}
A = \{ r \in \R^{3N} : \exists i,j \text{ such that }\hat x(r_i) = \hat x(r_j) \}
\end{equation}
has Lebesgue measure zero, and as defined in \Cref{eq:sortlet}, $\Psi_\alpha = \prod_{i=1}^N (\alpha_{i+1} - \alpha_i) = \pm \Psi_g$ on $\R^{3N} \backslash A$.
\end{proof}

\textbf{Remark:\\}
Since the expected value of any observable is independent of the sign of $\Psi$ (by linearity of the inner product the sign always cancels), this is enough to represent any ground state well enough to compute it's observables. Energy, which we've been discussing all along, is just the case where the observable is the Hamiltonian itself.
% To keep the logic tidy, we'll proceed in two separate steps: first we'll establish that an arbitrary (read: non-smooth) expansion of sortlets $\Psi_{\alpha}$ can represent $\Psi_g$, and then we'll show how we can smooth this expression using a tool from mathematical analysis known as mollification.

% \textbf{Arbitrary Representation:}\\
% Let $\Psi^g$ be a given antisymmetric function which integrates to unity ($\ang{\Psi_g | \Psi_g}$) and let $\beta^1 : \R^{3N} \longrightarrow \R^{N}$ be an arbitrary permutation equivariant function.  We'll define 
% \begin{equation}
% \label{eq:molly-alpha}  \alpha^1 = \begin{cases} \left[ {\text{sgn}[\Psi_g] \sigma(\pi_{\beta^1}) \vert \Psi_g \vert^{1/n} \over \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i})}\right]\beta^1  &\text{ : }  \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i}) \neq 0 \\ 0 &\text{ : } \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i}) = 0\end{cases}
% \end{equation}
% \jack{this assumes $N$ is odd, otherwise we might need complex roots of unity or some bs} proceeding by defining $\Psi_{\alpha^1} = \sigma (\pi_{\alpha^1})\prod_{i=1}^n (\alpha_{i+1} - \alpha_i )$ as before, then it follows
% \begin{equation}
%   \Psi_{\alpha^1}(x) = \Psi_g(x) \qquad \forall x \text{ such that } \prod_{i=1}^n (\beta^1_{i+1}(x) - \beta^1_{i}(x)) \neq 0
% \end{equation}

% by continuity, that the level set $A_1 = \{ x: \prod_{i=1}^n (\beta^1_{i+1}(x) - \beta^1_{i}(x)) = 0 \}$ forms an 3N - 1 dimensional hypersurface \cite{Lee2003}.  Continuing as one might expect, we next choose $\beta^2$ such that the set $A_2 \cap A_1$ has dimension 3N - 2. This can be accomplished by assuming the $\beta$ are all linear functionals, then $\beta_2 = \ang{\cdot, b_2}$ merely needs to be chosen such that $b_2$ is orthogonal to $b_1$. Venturing onward, we define $f_1 = \Psi_g - \Psi_{\alpha^1}$ and set 

% \begin{equation}
%   \alpha^2 = \begin{cases} \left[ {\text{sgn}[f_1] \sigma(\pi_{\beta^2}) \vert f_1 \vert^{1/n} \over \prod_{i=1}^n (\beta^2_{i+1} - \beta^2_{i})}\right] \beta^2  &\text{ : }  \prod_{i=1}^n (\beta^2_{i+1} - \beta^2_{i}) \neq 0 \\ 0 &\text{ : } \prod_{i=1}^n (\beta^2_{i+1} - \beta^2_{i}) = 0\end{cases}
% \end{equation}
% we now have 
% \begin{equation}
%   \Psi_{\alpha^1}(x) + \Psi_{\alpha^2}(x) = \Psi_g(x) \qquad \forall x \not \in A_1 \cap A_2
% \end{equation}
% Inductively, we can repeat this process for $\Psi_{\alpha^k}(x)$, reducing the dimension of the set where $\sum_{i=1}^k \Psi_{\alpha^i} \neq \Psi_g$ by 1 for each additional $k$. Max recursion depth is easily seen to be reached when $k = 3N$, in which case $A_1 \cap \cdots \cap A_{3N} = \varnothing$, and $\sum_{i=1}^{3N} \Psi_{\alpha^i} (x) = \Psi_g (x) : \forall x \in \R^{3N}$. 


% \begin{proof}
%    Let $r \in \R^{3N}$ be an arbitrary configuration, and choose $1 \leq i < j \leq N$ such that $r_i, r_j$ have the same spin. Define the transposition between these indices as $\tau$. For any $\pi \in S(N)$ that fixes $i, j$. We claim that $\tau \pi r$ is  in a different nodal cell than $r$. To see this, consider that the product comprising $\psipang$ contains a pairwise term $(\alpha_i - \alpha_j)$. Without loss of generality,  asume $\alpha_i(r) > \alpha_j(r)$. But for $\hat r = [\pi \tau]r$ we must have 
%    \begin{equation}
%     \left[ \phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\}) \right]= -  \left[ \phi_B(\hat r_i, \{\hat r\}) - \phi_B(\hat r_j, \{\hat r\}) \right]
%    \end{equation}
%    (because $\hat r_i = r_j$ and $\hat r_j = r_i$, and $\phi_B$ is otherwise invariant to $\pi r$).
%    Applying the intermediate value theorem (since $\Phi_B$ is assumed continuous), it then follows for any path 
%    \begin{equation} 
%     \gamma(t) : [0,1] \to \R^{3N} \qquad \gamma(0) = r \qquad \gamma(1) = \hat r
%    \end{equation}
%    connecting $r, \hat r$ must satisfy $\left[ \phi_B(\gamma(t')_i, \{\gamma(t')\}) - \phi_B(\gamma(t')_j, \{\gamma(t')\}) \right] = 0$ for some $t' \in (0,1)$. Again, since $\psipang = \prod_{i < j} \left[ \phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\}) \right]$, a zero in any term $\phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\})$ zeros $\Psi$. 
   
%    While a more thorough analysis could likely produce a tighter bound, an immediate consequence is that for systems of 4 or more electrons (with at least 2 spin up/down), there must be at least 4 nodal domains. This is because choosing $\pi$ to be a transposition of any other two electrons with the same spin yields that $\psipang(r)$ and $\psipang( \tau \pi r)$ must be in separate domains (note that the above holds for \textit{any} path interchanging $r, \tau \pi r$), despite having the same sign. Repeating the process from a different configuration $r'$ such that $\psipang$ has the opposite sign yields the same result. This implies there are at least two positive domains and two negative domains, for a minimum 4 total.
% \end{proof}



\textbf{Yeah, but isn't that expression like, horribly non-smooth?}\\
Actually, it's even worse than non-smooth, it's discontinuous. Luckily, functional analysis has produced a powerful technique we can wield to remedy this mess: \textit{mollifiers.} First, we'll define the standard mollifier as 
\begin{equation}
  \eta_\ep = \begin{cases}  c \exp{ {1 \over \vert x \vert^2 - 1} } : |x| < 1 \\ 0 : |x| \geq 1\end{cases}
\end{equation}
($c$ is just a constant chosen such that $\int \eta_\ep = 1$). If we then convolve an almost-everywhere differentiable $L_2$ function $f$ with $\eta_\ep$, we write $f^\ep := f \star \eta_\ep$. The power of this definition comes from the following properties of $f^\ep$ [see Section 4.2 in \cite{evans2015measure}]:
\begin{enumerate}
  \item $f^\ep$ is $C^{\infty}(\R^{3N})$, regardless of $f$.
  \item $f^\ep \to f$ in the sense that $\underset{\ep \to 0}{\lim} \Vert f - f_\ep \Vert_2 + \Vert \nabla f - \nabla f_\ep \Vert_2 = 0$ 
  %\item $f^\ep \to f$ pointwise, as $\ep \to 0$.
  %\item ${\partial f^\ep \over \partial x^i} \to {\partial f \over \partial x^i}$ where  ${\partial f \over \partial x^i}$ exists.
\end{enumerate}
% % Since ${\partial \Psi^{\alpha^k} \over \partial x^i}  = {\partial \Psi^g \over \partial x^i}$ for all $x \not \in A_1$, 
% Number 3 is the most relevant property for QMC purposes, since the idea is to solve for the ground state and then compute it's observables through integration. Energy, which we've been discussing all along, is just one of infinitely many possible observables. 

If we then set 
\begin{equation}
\alpha_\ep(r) = \left(\eta_\ep \star { |\Psi_g| \over \prod_{i=1}^N [x(r_{i+1}) - x(r_i)]}\right)^{1/n} x(r)
\end{equation}
we have that
\begin{equation}
\Psi_{\alpha^\ep} = \prod_{i=1}^{n} \left( \alpha^\ep_{i+1} - \alpha^\ep_{i} \right) = \eta_\ep \star  \left[{ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \right] \prod_{i=1}^n [\hat x(r_{i+1}) - \hat x(r_i)]
\end{equation}
It then follows that 
\begin{align}
    &\lim_{\ep \to 0} \Vert \Psi_\ep - \Psi_\alpha \Vert_2 \\
    = &\lim_{\ep \to 0} \left\Vert \left(\eta_\ep \star \left[{ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \right] - \left[{ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \right] \right)\prod_{i=1}^n [\hat x(r_{i+1}) - \hat x(r_i)] \right\Vert_2\\
    \leq &\lim_{\ep \to 0} \left\Vert \left(\eta_\ep \star \left[{ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \right] - \left[{ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \right] \right) \right\Vert_2 \sqrt{\pi}\\
    &= 0
\end{align}

Splitting up $\hat H = \nabla^2 + V$ (kinetic and potential), the proof of \Cref{thm:univ-energy} will follow directly from two propositions 

\begin{proposition}
\label{prop:kin-conv}
Assume ${ |\Psi_g| \over \prod_{i=1}^N [\hat x(r_{i+1}) - \hat x(r_i)]} \in W^{1,2}(\R^{3N})$. Then  
\begin{equation}
    \lim_{\ep \to 0} \ang{\Psi_{\alpha^\ep} | \nabla^2 | \Psi_{\alpha^\ep}} = \lim_{\ep \to 0} -\int_{\R^{3N}} [\nabla \Psi_{\alpha^{\ep}} \cdot \nabla \Psi_{\alpha^{\ep}}] = - \int_{\R^{3N}} \nabla \Psi_g \cdot \nabla \Psi_g
\end{equation}
\end{proposition}

\begin{proposition}
\label{prop:pot-conv}
Under the same assumption as \Cref{prop:kin-conv}, we have that 
\begin{equation}
\lim_{\ep \to 0} \ang{\Psi_{\alpha^\ep} | V | \Psi_{\alpha^\ep}} = \lim_{\ep \to 0}  \int_{\R^{3N}} V(x) \Psi_{\alpha^{\ep}}^2 = \int_{\R^{3N}} V(x) \Psi_g 
\end{equation}
\end{proposition}



% Let's define $\gamma^1 =\text{sgn}[f_1] \sigma(\pi_{\beta^2})$. We can easily show that ${\partial \gamma^1 \over \partial x^k}$ exists almost everywhere, since the discontinuous terms, $\text{sgn}[\Psi_g], \sigma(\pi_{\beta^1})$ are piecewise constant outside of the set $A = \bigcup_{k=1}^N A_k \cup \Psi^{-1}_g(\{0\})$. By the same argument as before, the $A_k$ and $\Psi_g^{-1}(0)$ are all null sets by virtue of being lower dimensional, so if we apply the standard mollifier by convolution to $\gamma^1$, we have that ${\partial (\gamma^1)^{\ep} \over \partial x^u} \to {\partial \alpha^1 \over \partial x^i}$ almost everywhere. By continuity on $\R^{3N} \backslash A$, we have that 
% \begin{equation}
%   \Psi_{(\alpha^1)^{\ep}} = \sigma(\pi_{\alpha^1})\prod_{i=1}^N [(\alpha^1_{i+1})^{\ep} - (\alpha^1_{i})^{\ep}] \to \prod_{i=1}^N [(\alpha^1_{i+1}) - (\alpha^1_{i})] = \Psi_{\alpha^1}
% \end{equation}
% pointwise.  

\begin{proposition}
  Let $\Psi$ be $\psi'_{\text{pair}}$ as defined in \eqref{eq:pairwise}. Then $\Psi$ has at least $n(n-1)/2$ nodal domains. Since the ground state is proven to have only 2 for Li, Be, (and conjectured to in general), this implies one Vandermonde determinant is insufficient to accurately represent the ground state.
\end{proposition}
\begin{proof}
   Let $r \in \R^{3N}$ be an arbitrary configuration, and choose $1 \leq i < j \leq N$ at will. Define the transposition between these indices as $\tau$. For any $\pi \in S(N)$ that fixes $i, j$. We claim that $\tau \pi r$ is  in a different nodal cell than $r$. To see this, consider that the product comprising $\Psi_1$ contains a pairwise term $(\alpha_i - \alpha_j)$. Without loss of generality, for $\Psi_1(r)$, we have $\alpha_i(r) > \alpha_j(r)$. But for $\hat r = \pi \circ \tau (r)$ we must have 
   \begin{equation}
    \left[ \phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\}) \right]= -  \left[ \phi_B(\hat r_i, \{\hat r\}) - \phi_B(\hat r_j, \{\hat r\}) \right]
   \end{equation}
   (because $\hat r_i = r_j$ and $\hat r_j = r_i$, and $\phi_B$ is assumed invariant to $\pi$).
   Applying the intermediate value theorem (since $\Phi_B$ is assumed continuous), it then follows for any path 
   \begin{equation} 
    \gamma(t) : [0,1] \to \R^{3N} \qquad \gamma(0) = r \qquad \gamma(1) = \hat r
   \end{equation}
   connecting $r, \hat r$ must satisfy $\left[ \phi_B(\gamma(t')_i, \{\gamma(t')\}) - \phi_B(\gamma(t')_j, \{\gamma(t')\}) \right] = 0$ for some $t' \in (0,1)$. Again, since $\Psi = \prod_{i < j} \left[ \phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\}) \right]$, a zero in any term $\phi_B(r_i, \{r\}) - \phi_B(r_j, \{r\})$ zeros $\Psi$.
\end{proof}
Importantly, since $\pi$ was arbitrary, this prohibits the sort of triple exchanges \cite{mitas2006fermion} which in the exact ground state, connect same sign regions and collapse the number of nodal cells to 2. 


% We are now ready to state and prove the following theorem:

% \begin{corollary}
%   We can approximate the ground state energy, $E = \ang{\Psi_g \vert H \vert \Psi_g}$ arbitrarily well with a sequence of sorting ansatz $\Psi^\ep$, via the sequence $E_\ep = \ang{\Psi^\ep \vert H \vert \Psi^\ep}$
% \end{corollary}
% \begin{proof}
% Without loss of generality, we first decompose $O$ as a sum of terms, $O = \sum_i O_i$, where the highest degree of a partial appearing in $O_i$ is at most $i$. The proof will then follow from applying the dominated convergence theorem to the integrals
% \begin{equation}
%   \ang{\Psi^\ep | O_i | \Psi^\ep} = \int_{\R^{3N}} \Psi^\ep(x) [O_i \Psi^\ep](x) dx
% \end{equation}
% to do this, we first need to show that the integrand, $\Psi^\ep [O_i \Psi^\ep]$, is dominated by $\Psi_g [O_i \Psi_g]$. We'll begin by showing $\Psi^\ep < \Psi_g$ almost everywhere. Unrolling the definition of $\Psi^\ep$, we find 

% \begin{align*}
%   \vert \Psi^\ep \vert &= \left \vert \sigma(\pi_{\alpha^1})\prod_{i=1}^N [(\alpha^1_{i+1})^{\ep} - (\alpha^1_{i})^{\ep}] \right \vert \\ 
%   &= \sigma(\pi_{\alpha^1}) \prod_{i=1}^N   \vert \Psi_g \vert^{1/n}  \left[ { \vert   \eta_\ep \star (\text{sgn}[\Psi_g] \sigma(\pi_{\beta^1})) \vert \over \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i})} \left( \beta^{i+1} - \beta_i \right) \right] \\ 
%   &\leq  \vert \Psi_g \vert \prod_{i=1}^N  \left[{  1 \over \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i})} \left( \beta^{i+1} - \beta_i \right) \right] \tag{ a.e }\\
%   &= { \vert \Psi_g \vert \over \prod_{i=1}^n (\beta^1_{i+1} - \beta^1_{i}) } \prod_{i=1}^N  \left( \beta^1_{i+1} - \beta^1_i \right)  = \vert \Psi_g \vert \tag{a.e}
% \end{align*}
% Note the immediate consequence that $\ang{\Psi^\ep | O_0 | \Psi^\ep} \to \ang{\Psi_g | O_0 | \Psi_g}$.
% \end{proof}



\textbf{Discussion (why use more than one sortlet then?):}\\
% A natural reaction to the form of [eqref] might be to ask, do we really need more than one term? Since all we care about is the energy, which is an average over $\R^{3N}$, it might seem tempting to conclude that we only need to approximate $\Psi_g$ up to a set of measure 0, which is achieved with just 1 term. Practically, however, it's important to remember that since that expression is non-smooth, yet our $\alpha$ are always smooth, it's not so similar. \jack{this is bs} Intuitively, one can see that since the set $A_1^\ep$ is $\ep$ thick, and decreasing $\ep$ will likely require increasing the norm of our parameters since it naturally, inversely corresponds to a notion of "smoothness." Adding more terms reduces the volume of the set $E_k = \bigcap_{i=1}^k A_k^\ep$ exponentially, which practically means a much better fit of $\Psi_g$, at least as far as the energy is concerned.



==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

